Can phase change materials in building insulation improve self-consumption of residential rooftop solar? An Australian case study

This work investigates the extent to which phase change material (PCM) in the building's envelope can be used as an alternative to battery storage systems to increase self-consumption of rooftop solar photovoltaic (PV) generation. In particular, we explore the electricity cost-savings and increase in PV self-consumption that can be achieved by using PCMs and the operation of the heating, ventilation, and air conditioning (HVAC) system optimised by a home energy management system (HEMS). In more detail, we consider a HEMS with an HVAC system, rooftop PV, and a PCM layer integrated into the building envelope. The objective of the HEMS optimisation is to minimise electricity costs while maximising PV self-consumption and maintaining the indoor building temperature in a preferred comfort range. Solving this problem is challenging due to PCM's nonlinear characteristics, and using methods that can deal with the resulting non-convexity of the optimisation problem, like dynamic programming is computationally expensive. Therefore, we use multi-timescale approximate dynamic programming (MADP) that we developed in our earlier work to explore a number of Australian PCM scenarios. Specifically, we analyse a large number of residential buildings across five Australian capital cities. We find that using PCM can reduce annual electricity costs by between 10.6% in Brisbane and 19% in Adelaide. However, somewhat surprisingly, using PCM reduces PV self-consumption by between 1.5% in Brisbane and 2.7% in Perth.

==> fig-ANN-trans-fxn-approximator.tex <==
\begin{figure}
	\centering
	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
	\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1,scale=0.70,every node/.style={scale=0.90}]
		%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300
		
		%Rounded Rect [id:dp7683821390135787] 
		\draw   (241,122.7) .. controls (241,110.77) and (250.67,101.1) .. (262.6,101.1) -- (356.9,101.1) .. controls (368.83,101.1) and (378.5,110.77) .. (378.5,122.7) -- (378.5,187.5) .. controls (378.5,199.43) and (368.83,209.1) .. (356.9,209.1) -- (262.6,209.1) .. controls (250.67,209.1) and (241,199.43) .. (241,187.5) -- cycle ;
		%Straight Lines [id:da7740597204378653] 
		\draw    (143.5,110) -- (240.5,110.97) ;
		\draw [shift={(243.5,111)}, rotate = 180.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.5,-6.01) -- (0,0) -- (12.5,6.01) -- cycle    ;
		%Straight Lines [id:da5836445613152903] 
		\draw    (141.5,140) -- (238.5,140.97) ;
		\draw [shift={(241.5,141)}, rotate = 180.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.5,-6.01) -- (0,0) -- (12.5,6.01) -- cycle    ;
		%Straight Lines [id:da3876429356636124] 
		\draw    (140.5,170) -- (237.5,170.97) ;
		\draw [shift={(240.5,171)}, rotate = 180.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.5,-6.01) -- (0,0) -- (12.5,6.01) -- cycle    ;
		%Straight Lines [id:da06968422702484367] 
		\draw    (144.5,197) -- (241.5,197.97) ;
		\draw [shift={(244.5,198)}, rotate = 180.57] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.5,-6.01) -- (0,0) -- (12.5,6.01) -- cycle    ;
		%Straight Lines [id:da8996169498906234] 
		\draw    (379.75,152.1) -- (472.5,152) ;
		\draw [shift={(475.5,152)}, rotate = 539.94] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.5,-6.01) -- (0,0) -- (12.5,6.01) -- cycle    ;
		
		% Text Node
		\draw (295,145) node [anchor=north west][inner sep=0.75pt]   [align=left] {ANN};
		% Text Node
		%\draw (120,121) node [anchor=north west][inner sep=0.75pt]    {$$};
		% Text Node
		\draw (151,121) node [anchor=north west][inner sep=0.75pt]    {$T_{in,k-1}$};
		% Text Node
		\draw (151,150) node [anchor=north west][inner sep=0.75pt]    {$T_{out,k-1}$};
		% Text Node
		\draw (151,178) node [anchor=north west][inner sep=0.75pt]    {$T_{out,k} \ $};
		% Text Node
		\draw (151,95) node [anchor=north west][inner sep=0.75pt]    {$x_{k}$};
		% Text Node
		\draw (399,133) node [anchor=north west][inner sep=0.75pt]    {$T_{in,k}$};
	\end{tikzpicture}
	\vspace{0.2cm}
	\caption{The ANN transition function approximator. The ANN has four inputs, including HVAC system status (on/off), the indoor temperature at $k-1$, $T_{\text{in},k-1}$, the outdoor temperature at $k$, $T_{\text{out},k}$, the outdoor temperature at $k-1$, $T_{\text{out},k-1}$, while the output is the indoor temperature at $k$, $T_{\text{in},k}$.}
	\vspace{-0.2cm}
	\label{fig:NN}
\end{figure}
